YAMLE: Yet Another Machine Learning Environment

YAMLE: Yet Another Machine Learning Environment is an open-source framework that facilitates rapid prototyping and experimentation with machine learning (ML) models and methods. The key motivation is to reduce repetitive work when implementing new approaches and improve reproducibility in ML research. YAMLE includes a command-line interface and integrations with popular and well-maintained PyTorch-based libraries to streamline training, hyperparameter optimisation, and logging. The ambition for YAMLE is to grow into a shared ecosystem where researchers and practitioners can quickly build on and compare existing implementations. Find it at: https://github.com/martinferianc/yamle.

==> outline.tex <==

\author{\name Martin Ferianc$^{1}$ \email martin.ferianc.19@ucl.ac.uk \\
\name Miguel Rodrigues$^{1}$ \email m.rodrigues@ucl.ac.uk \\
\addr $^{1}$Department of Electronic and Electrical Engineering\\
University College London}

\section{Introduction}\label{sec:introduction}
\begin{itemize}
    \item Background and motivation for building the library
    \item The significance of open-source machine learning libraries
    \item Purpose and scope of the paper
\end{itemize}

\section{Library Overview}\label{sec:library-overview}
\begin{itemize}
    \item Name and version of the library
    \item Brief description of the library's functionality
    \item Key features and capabilities
    \item Target audience and user base
\end{itemize}

\section{Design and Architecture}\label{sec:design-architecture}
\begin{itemize}
    \item High-level architectural overview
    \item Explanation of the design principles and decisions
    \item Supported programming languages and platforms
    \item Integration with other libraries and frameworks
\end{itemize}

\section{Core Components and Modules}\label{sec:core-components-modules}
\begin{itemize}
    \item Detailed breakdown of the library's core components
    \item Description of key modules and their functions
    \item Examples of how to use the library for common tasks
\end{itemize}

\section{Performance and Efficiency}\label{sec:performance-efficiency}
\begin{itemize}
    \item Benchmarking results (if available)
    \item Discussion of optimization techniques used
    \item Scalability considerations
\end{itemize}

\section{Documentation and Support}\label{sec:documentation-support}
\begin{itemize}
    \item Availability and completeness of documentation
    \item User guides, tutorials, and examples
    \item Community support, forums, and resources
\end{itemize}

\section{Use Cases and Applications}\label{sec:use-cases-applications}
\begin{itemize}
    \item Real-world applications of the library
    \item Success stories or case studies
    \item Testimonials from users (if available)
\end{itemize}

\section{Future Development and Roadmap}\label{sec:future-development-roadmap}
\begin{itemize}
    \item Planned enhancements and features
    \item Community contributions and collaboration opportunities
    \item Versioning and release strategy
\end{itemize}

\section{Comparisons with Existing Libraries}\label{sec:comparisons-existing-libraries}
\begin{itemize}
    \item Comparison with similar open-source libraries
    \item Advantages and unique selling points of your library
\end{itemize}

\section{Conclusion}\label{sec:conclusion}
\begin{itemize}
    \item Summary of the library's key contributions
    \item Reiteration of its importance in the machine learning ecosystem
    \item Encouragement for readers to explore and contribute to the library
\end{itemize}


\section{Core Components and Modules}\label{sec:core-components-modules}
\begin{itemize}
    \item YAMLL is built on PyTorch and PyTorch Lightning.
    \item In contrast to other libraries, YAMLL opted for PyTorch thanks to its popularity and ease of use which makes it a good choice for a general-purpose machine learning library. Additionally, PyTorch Lightning~\citep{falcon2019pytorch} already saves a lot of boilerplate code and provides a standardised interface for training models including the optimisation and evaluation. Moreover, the library relies on torchmetrics~\citep{torchmetrics} for evaluation metrics and syne-tune~\citep{salinas2022syne} for hyperparameter optimisation.
    \item The library is divided into three main components - `DataModule`, `Model` and `Method` - which are infrastructurally connected but can be independently modified and extended.
    \begin{itemize}
        \item `DataModule`, defined in `yamll/data/datamodule.py' 
        is responsible for downloading, loading and preprocessing data. 
        \item It also defines the task which is going to be solved by the `Method` and `Model`.
        \item It handles the data splitting into training, validation and test sets.
        \item The `DataModule` needs to be subclassed for any additional dataset or task to be solved.
    \end{itemize}
    \begin{itemize}
        \item `Model`, defined in `yamll/models/model.py' is responsible for defining the architecture of the model.
        \item It defines the forward pass of the model.
        \item It has to define several components e.g. the `_input' and `_output' layers which can be modified by the `Method`.
        \item The `Model` needs to be subclassed for any additional model to be used.
    \end{itemize}
    \begin{itemize}
        \item `Method`, defined in `yamll/methods/method.py' is responsible for defining the interface that can optionally change the model and defines the training, validation and test steps by reusing the functionality provided by PyTorch Lightning.
        \item E.g. `Method' can be used to implement a new training algorithm through overloading the `_training_step`, `_validation_step` and `_test_step` methods.
        \item It also takes into account the loss function, optimiser and any regularisation during training.
        \item It also can take into account `Pruning` followed by `Quantisation' during evaluation.
        \item Through callbacks it enables logging and reporing of the metrics to the user or the Hyperparameter Optimisation.
        \item The `Method` needs to be subclassed for any additional method to be used.
    \item The `DataModule', `Model` and `Method` enable customisation through defining their own arguments that can be triggered via `argparse`
    \item All the components are grouped together by `Trainer/Tester' which is responsible for querying the `DataModule', `Model' and `Method' and running the training and evaluation through the `_training_step`, `_validation_step` and `_test_step` methods as well as running on a specific device platform.
    \item All classes are already connected and enable end-to-end experiments from data preprocessing to model training and evaluation.
    It is necessary just to sublass the right classes, register them in the framework such that they can be selected through `argparse' and run the training or evaluation via the methods defined in `yamll/cli`.
\end{itemize}

\section{Use Cases and Applications}\label{sec:use-cases-applications}
\begin{itemize}
    \item The library is not meant to be used as an addon to an existing project but as the main project itself.
    \item For example, the user wants to propose a new machine learning method or model and wants to compare it to existing methods and models.
    \item 1. The user experiments with the new method or model by subclassing the \texttt{Method} or \texttt{Model} on the \texttt{DataModule} of choice.
    \item 2. When the user is satisfied with the results the user submits a pull request to the library.
    \item 3. The pull request will be reviewed and the new feature will be added to the library.
    \item This means that everyone else can use the new method or model and compare it to other methods and models.
    \item This in contrast to the current situation where everyone implements their own version of the method or model in their own repository in which they provide a custom implementation of all additional components which should not be necessary.
    \item There are three main use cases:
    \begin{itemize}
        \item \textbf{Training}: which can be done by running \texttt{python -m yamll/cli/train.py} e.g. with:
        \begin{itemize}
            \item \texttt{python3 yauq/cli/train.py --method base --trainer_devices "[0]" --data mnist --data_batch_size 256 --method_optimizer adam --method_learning_rate 3e-4 --regularizer l2 --method_regularizer_weight 1e-5 --loss crossentropy  --save_path ./experiments --data_pad_to_32 1 --trainer_epochs 3 --model_hidden_dim 32 --model_depth 3 --data_val_portion 0.1 --save_path ./experiments}
            \item This is a simple example of training a multi-layer perceptron on the MNIST dataset.
        \end{itemize}
        \item \textbf{Testing}: which can be done by running \texttt{python -m yamll/cli/test.py} e.g. with:
        \begin{itemize}
            \item \texttt{python3 yauq/cli/test.py --method base --trainer_devices "[0]" --data mnist --data_batch_size 256 --save_path ./experiments --data_pad_to_32 1 --model_hidden_dim 32 --model_depth 3 --data_val_portion 0.1 --load_path ./experiments/<FOLDER>}
            \item This is a simple example of testing a multi-layer perceptron on the MNIST dataset.
        \end{itemize}
        \item \textbf{Hyperparameter Optimization}: which can be done by running \texttt{python -m yamll/cli/tune.py} e.g. with:
        \begin{itemize}
            \item \texttt{python3 yauq/cli/tune.py --config_file <FILE.py> --optimizer "Grid Search" --save_path ./experiments/hpo/ --max_wallclock_time 420 --optimization_metric "val_nll"}
            \item This is a simple example of grid search depending on the specified config file defining the search space as per syne-tune's documentation.
        \end{itemize}
    \item Therefore, the user can easily train, test and optimize hyperparameters of the model or method covering the whole pipeline from data preprocessing to model training and evaluation.
    \end{itemize}
\end{itemize}
